Can Intelligent Hyperparameter Selection Improve Resistance to Adversarial Examples?

Convolutional Neural Networks and Deep Learning classification systems in general have been shown to be vulnerable to attack by specially crafted data samples that appear to belong to one class but are instead classified as another, commonly known as adversarial examples. A variety of attack strategies have been proposed to craft these samples; however, there is no standard model that is used to compare the success of each type of attack. Furthermore, there is no literature currently available that evaluates how common hyperparameters and optimization strategies may impact a model's ability to resist these samples. This research bridges that lack of awareness and provides a means for the selection of training and model parameters in future research on evasion attacks against convolutional neural networks. The findings of this work indicate that the selection of model hyperparameters does impact the ability of a model to resist attack, although they alone cannot prevent the existence of adversarial examples.

==> attackModel.tex <==
\chapter{Adversarial Influence of Neural Networks}
\label{sec:influence}


The attack surface of a machine learning model is highly dependent on the implementation details of the system that is using the model. The model itself can only be modified directly by an adversary that has compromised the system it resides in or indirectly by an adversary that can influence the data that is used to either train or update the model. The direct modification of a machine learning model is only possible when the infrastructure which the model resides in is compromised. In this situation, we assume that the adversary has complete control of the model and can manipulate the learned parameters of the model to reach their goal. An indirect attack is slightly different in that it relies more on the way a system collects and trains on data. There are a variety of potential avenues for attack depending on these factors, but these same system design decisions may also lead to constraints on an adversary. These factors and their impact on adversarial influence of a CNN are discussed in the following sections.

\section{Attack Modeling}
\label{sec:modeling}

Biggio et al.\cite{biggio_security_2014-1}  present a formal method for describing an attack scenario on a classifier systems. This methodology provides a baseline for defining the potential causative attacks against CNNs. The description of a scenario in this framework is split into four components; the adversary's goal, knowledge, capability, and strategy. The following sections explain these components in the context of causative attacks on CNNs.

\subsection{Adversary Goals}
\label{model:goals}

The taxonomy presented by Huang et al.\cite{huang_adversarial_2011}  explains the objective of the adversary, described by the security violation and the attack specificity that is intended.

\subsection{Adversary Knowledge}
\label{model:knowledge}

The knowledge available to the adversary about the CNN. This includes initial knowledge about the algorithm design as well as knowledge that the adversary can acquire through interactions with the model. The knowledge described in this framework includes:

\begin{itemize}
	\item Training Data
	\item Feature Set
	\item Network Parameters and Feature Weights
	\item Feedback from the Classifier
\end{itemize}

%what about knowledge of the system

\subsection{Adversary Capability}
\label{model:capability}

The influence over the training and testing data. Because this work is focused on targeted attacks, we are only interested in our impact on the training data. Other capabilities the attacker may have include the ability of the adversary to affect the class priors, the percentage of data that can be manipulated, and to what degree in which that data may be manipulated.

%what about test data and causing drift?

\subsection{Adversary Strategy}
\label{model:strategy}

The final component of the attack scenario is a definition of the optimal attack strategy based on the goal, knowledge, and capability of an adversary. This strategy describes how an attack is carried out, including how data is manipulated and to what extent it is changed, as well as any other actions that an attacker takes during the attack.
%e.g....example

\section{Variables Impacting the Attack Model}
\label{sec:attackVars}

Each component of the described attack model can be influenced by both internal and external variables of the learning system. Internal variables include the aspects of the system that are under control of the operator of the system, including processes such as data collection and decisions such as model parameters. External variables include all other factors that are not controlled by the operator of the system, such as concept drift in the underlying environment. In this section, these two types of variables are described along with the security impact that they may have on a learning system.

\subsection{Internal Variables}
\label{vars:internal}

Internal stimuli are defined as the decisions or variables of a machine learning system that impact its potential attack models and which are under control by an operator of that system. Although they are controlled by the operator of the system, choosing whether to include these stimuli and what their values are is not always a straightforward process. Many times, this decision includes a tradeoff between the security of the resulting model and its performance or usability. This has been discussed in []. To understand how to build a secure application that utilizes a CNN model, understanding these various stimuli and how they impact the security of the resulting model is important when examining this tradeoff. In some cases, the inclusion or change in value of one of these stimuli could lead to a more powerful attack model, or a system that is easier to compromise. In this case, it may be reasonable to accept the performance tradeoff for a more secure model. On the other hand, if the performance of the model suffers too much from, the system may be unusable. In this section, the various types of internal stimuli are discussed in the context of CNNs.

\subsubsection{Algorithm}

The tradeoff between performance and security is most relevant in the decisions around the hyperparameters of a CNN. The selection processes for hyperparameters generally strive to increase the performance of the outputted model, but little work has been done to understand how these parameters impact an adversary’s ability to manipulate the model given any control over the training data. One can imagine that parameters such as learning rate could change the influence that even a small amount of malicious training data may exert over the resulting model. Other parameters of a CNN that may influence an adversary’s capability include the number of layers in, number of units per layer, the type of activation function used, momentum, regularization, and optimization weights.

\subsubsection{Application}

The decisions surrounding the requirements and functionality of the application that uses the model can influence the knowledge and capability of an attacker. Some of the decisions around functionality of an application may be impossible to leave out, such as a response mechanism for a CNN that is responsible for detecting cancer in an image. This is a central feature required for the application to function, but it does provide an adversary with an oracle\cite{?} that provides more knowledge about the model. In some cases, this functionality may be an extraneous feature, such as in a pervasive setting in which the output of a model is not relayed back to the world and is only used to make an internal decision about the state of the world. An example of this could be a system that detects behavior patterns in humans and uses this knowledge to make other decisions at a higher level. For example, a feedback mechanism in this system may be interesting and useful for debugging, but would be unnecessary for the application to function and furthermore adds to the knowledge of the adversary. Other internal security stimuli in an application may include the lack of access permissions to the output or data in an application, the ability to query the application in real time, and the ability to send training data to the system such as in a crows sensing system.

\subsubsection{Defense}

The primary purpose of a defense mechanism should be to limit some or all components of an attack model in order to make it difficult or impossible to achieve the attacker’s goal. This is generally done by adding constraints of some type to either the training data or to the resulting model. For example, the Reject on Negative Impact(RONI)\cite{}  defense keeps multiple copies of a model so that if a batch of training data has a negative impact on the performance of the resulting model, it is rejected and the old model is used. This adds the constraint to the attacker’s capability such that they may not impact the model enough to cause a decrease in the performance of the classifier with the new training data, and prevents an attacker from reaching the goal of poor performance. However, other attacks such as a simple denial of service on new training data, or a boiling frog attack\cite{huang_adversarial_2011} are still possible. Other defenses that have been explored included anomaly detection, adversarial training, game-theoretic approaches, and robust learning mechanisms.\cite{}

%not controlled internally \subsubsection{environment}

\subsubsection{Features and Structure of Data}

The impact of features and structure of a data set are largely an external matter. However, the extraction of features from the data is controlled by the system designer. Variables such as the number of features and the importance of each of these features can constrain the capability of an attacker. As more features are collected from a set of data such as a picture, it may be difficult for an adversary to find and modify those features.

\subsubsection{Learning Process}

The process in which a learning system creates and updates a model influences the capability of an attacker and the strategy they may use to reach their goal. As new information is collected for a model, the response of the system and the mechanism employed to train on this new data can change the potential avenues for attack. For instance, if malicious data is added to the training data of a CNN, the influence exerted over the resulting model may vary depending on whether the model is updated or trained from scratch with the new data. Other important factors in the learning process with respect to security include the length of time that old training data is held and the triggering mechanism for a model update. 

%\subsubsection{State of model under Attack}
\subsubsection{Human Analysis}
%\subsubsection{Attacker's Access}

When a human analyst is reviewing the model and data, there is the added constraint on any new malicious samples in the training data and on the performance of the resulting model. This constraint is largely dependent on what level the analyst is reviewing the model at. For example, an analyst could choose to sample new training data spot check the accuracy of their labels, which may limit the feasibility of certain attacks such as a label flipping attack\cite{biggio14-neurocomp}. However, this takes a significant amount of time and effort and may be impossible. In a more likely example, a human analyst may review the learning curves of higher level metrics to determine if the model is performing well. The constraint added by this type of analysis depends on the metrics that are used for analysis.

\subsection{External Variables}
\label{vars:external}

External Stimuli are defined in this work as the variables in the implementation of a machine learning system that impact its attack model and which are not under control of the operator of the system. These variables are important to the attack model in the same way as the internal variables of the system, i.e. they can either limit or enhance an adversary’s ability to influence the system. In the case of most systems, this impact is limited to the natural structure of the information that is collected and the underlying environment that is creating the data. Since no control can be exerted over these variables, the system design must account for their presence and the operator must understand the impact that they have on the security of the model.

%\subsubsection{Application}
%\subsubsection{Defense}
\subsubsection{Environment}

Various properties of the underlying environment that produces the data that the system learns on influence the way that the system responds to an attack. The system must adapt to this environment, so any changes in the environment, or concept drift, change the way that the learning process occurs. This adds the requirement to the system that it must be able to adapt to this drift, which also means it must continue to collect new data from the environment. This new data could be malicious, and because the system must learn new drift, the adversary also has a new attack strategy of either “triggering” this drift to occur when it is not occurring through the introduction of false drift or influencing the speed with which the drift occurs. Also of interest is the number of adversaries in the environment as well as the amount of control that they may exert over new data.

Other potential impacts that the environment may have on the attack model include the rate at which data is produced for each class and the introduction of new labels in an environment, and simply the amount of data that has been produced overall to train on. These variables can impact both the performance of a model (when there is not enough training data that represents the current environment) and the security of the model, making it more prone to causative attacks.


\subsubsection{Features and Structure of Data}

The structure of the data that is collected for training with a CNN can impact the level of corruption of the training data that is required for an adversary to accomplish their goal. Depending on the training data, certain features may be far more important than others. If there are only a small number of important features, it may be easier for an adversary to cause one class to be mislabeled as another. Likewise, if the feature values of two classes are similar, it may be easier to cause a shift in the classification of those two classes. For example, a CNN that classifies bowling balls and pool balls may have a weakness due to similar features the two. On the other hand, the features of humans and turtles are likely very different, and poisoning a model that does that classification may be more difficult.

%\subsubsection{Learning Process}
%\subsubsection{State of Model Under Attack}
%\subsubsection{Human Analysis}
%\subsubsection{Attacker's Access}

\section{Defining Attack Strategies}
\label{sec:definingAttack}

\section{Types of Strategies}
\label{sec:strategyTypes}

\section{Setting Up the Problem}
\label{sec:problemSetup}


==> related.tex <==
\chapter{Related Work}
\label{sec:related}

\section{Exploratory Attacks}

\section{Causative Attacks}

\section{Defenses}

\subsection{Game-theoretic}

\subsection{Robust Learning}



==> secureDesign.tex <==
\chapter{Designing DNNs to Withstand Attacks}
\label{sec:secDesign}


